Differentially Private Nonparametric Hypothesis Testing

Hypothesis tests are a crucial statistical tool for data mining and are the workhorse of scientific research in many fields. Here we study differentially private tests of independence between a categorical and a continuous variable. We take as our starting point traditional nonparametric tests, which require no distributional assumption (e.g., normality) about the data distribution. We present private analogues of the Kruskal-Wallis, Mann-Whitney, and Wilcoxon signed-rank tests, as well as the parametric one-sample t-test. These tests use novel test statistics developed specifically for the private setting. We compare our tests to prior work, both on parametric and nonparametric tests. We find that in all cases our new nonparametric tests achieve large improvements in statistical power, even when the assumptions of parametric tests are met.

==> Algorithms.tex <==
\section{Algorithms}\label{sec:algos}

% WC -------------------------------------------------------------

% KW -------------------------------------------------------------
\subsection{Traditional Kruskal-Wallis}

In this section, we assert a bound on the sensitivity of the $\statsqu$-statistic, outline our algorithm for the private Kruskal-Wallis, and prove that the algorithm is $\epsilon$-differentially private. We then present a complete algorithm for calculating a p-value and prove that it too is $\epsilon$-differentially private. 

\begin{theorem} \label{thm:squaresensi}
The sensitivity of $\statsqu$ is bounded by 87.
\end{theorem}

See Appendix \ref{sec:kw_sq_sens} for a proof of Theorem \ref{thm:squaresensi}.

For a database $\data$, our algorithm begins by adding a small amount of random noise to each data point to randomly order any ties (this allows us to use the simpler version of the $\statsqu$ formula, and thus the above bound on the sensitivity). We may then compute the $\statsqu$-statistic as in the public setting and add noise proportional to the sensitivity.

\begin{algorithm}[!htb]
\DontPrintSemicolon
\algrule
\textbf{Algorithm} $\privKW$ \textbf{:} Differentially Private Kruskal-Wallis Statistic\;
\algrule
\KwIn{$\data$, $\epsilon$}
\Begin{
    \For{all data points $i$ in \data}{
        $i = i \ +$ small noise \;
    } 
    $\statsqu \longleftarrow \KW(\data)$\;
    $\widetilde{\statsqu} \longleftarrow \statsqu + \lap \Big (87/\epsilon \Big )$\;
}
\KwOut{$\widetilde{\statsqu}$}
\algrule 
\end{algorithm}

\begin{theorem} \label{thm:pKW}
    Algorithm $\privKW$ is $\epsilon$-differentially private.
\end{theorem}

\begin{proof}
There are two sources of randomness inside Algorithm $\privKW$: the noise added to break ties and the Laplace mechanism. So let us write $\privKW(\data) := \privKW(\data;r_1,r_2),$ where $r_1$ indicates the randomness of breaking ties and $r_2$ indicates the randomness of the Laplace noise added to $\KW(\data)$. Let $r_1^*$ be a fixed way to sort ties, and $r_1^*$ be a random choice of $r_1$. 

Consider $\privKW_{r_1^*}(\data;r_2)$, which modifies $\data$ using $r_1^*$ to break ties, then calculates the test statistic $h$ of the modified $\data$. It then outputs $\widetilde{\statsqu} = \statsqu + \lap \Big (87/\epsilon \Big )$, where $87$ is the global sensitivity computed in Appendix \ref{sec:kw_sq_sens}. $\privKW_{r_1^*}(\data;r_2)$ is simply a Laplace mechanism, so $\epsilon$-differential privacy follows by Theorem \ref{thm:lm}.

Then as $r_1^*$ is a random choice of $r_1$, $\privKW_{r_1^*}(\data;r_2)$ can be seen as a random choice of $\privKW(\data;r_1,r_2)$. Since $\privKW_{r_1^*}(\data;r_2)$ is $\epsilon$-differentially private, $\privKW(\data;r_1,r_2)$ is also $\epsilon$-differentially private. Therefore Algorithm $\privKW$ is $\epsilon$-differentially private.
\end{proof}

\begin{algorithm} [!htb]
\DontPrintSemicolon
\algrule
\textbf{Algorithm} $\complete$ \textbf{:} Complete Kruskal-Wallis Test\;
\algrule
\KwIn{\data, $\epsilon$, $c$}
\Begin{
	$\widetilde{\statsqu} := \privKW(\data, \epsilon)$\;
	$g \longleftarrow $ the number of groups of $\data$\;
    \For{$k := 1$ \textup{to} $c$}{
        $\data^* \longleftarrow $ a database with $g$ groups generated under $H_0$\;
        $h_k \longleftarrow \privKW(\data^*)$;
    }
    $p \longleftarrow$ fraction of $h_k$ more extreme than $\tilde{\statsqu}$ \;
}
\KwOut{$\widetilde{\statsqu}, p$}
\algrule
\label{alg:complete_kw}
\end{algorithm}

Algorithm $\complete$ gives our complete algorithm to find a p-value given a database $\data$, privacy parameter $\epsilon$ and number of repetitions $c$. It begins by calculating the private $h$-test statistic of database $\data$. It then generates $c$ databases $\data^*$ under $H_0$ with $g$ groups, each with $\lfloor\frac{n}{g}\rfloor$ elements (determined such that the sum of the groups is less than or equal to $n$). The test statistic $h_k$ for each of these databases is then computed\footnote{When we use the traditional Kruskal-Wallis test, the distribution of $h$-statistics asymptotically converges to the $\chi^2$ distribution. Thus, for efficiency purposes, we take $H_k \sim {\sf \chi^2}(g-1) + \lap(\Delta \statsqu/\epsilon)$}. The p-value is the percent of $h_k$ more extreme than $h$. See Appendix \ref{sec:kw_sq_t1} for a note on the Type I error rate of $\complete$.

%Inside the for loop of Algorithm $\complete$, $\data^*$ is a database generated under $H_0$. It contains $g$ groups and each group contains roughly $N/g$ numbers of data (sum to $N$) and they all come from the same distribution \footnote{For efficiency purposes, when we use the traditional Kruskal-Wallis test, as asymptotically the distribution of $h$-statistics converge to $\chi^2$ distribution, we can calculate $h_k$ by $h_k \longleftarrow {\sf \chi^2}(g-1) + \lap(\Delta \statsqu/\epsilon)$}.

\begin{theorem} \label{thm:pcomp}
Algorithm $\complete$ is $\epsilon$-differentially private.
\end{theorem}

\begin{proof}
By Theorem \ref{thm:pKW}, the computation of $\tilde{\statsqu}$ is $\epsilon$-differentially private. All of the following steps, generating the reference distribution and calculating $p$-value do not need to access to the database $\data$, and therefore by Theorem \ref{thm:pp} (post processing), Algorithm $\complete$ is $\epsilon$-differentially private.
\end{proof}


% KW -------------------------------------------------------------
\subsection{Absolute Value Kruskal-Wallis}

In this section, we follow the example of \simon{This should reference the new ANOVA paper.} and introduce a variant of the Kruskal-Wallis, where the squares in the formula are replaced with absolute values, making the statistic 
$$\statabs = (n - 1) \frac{\sum_{i=1}^g n_i | \bar{r}_i - \bar{r} | }{\sum_{i=1}^g \sum_{j=1}^{n_i} | r_{ij} - \bar{r} | }.$$

As before, when there are no ties in the data, the statistic can be reduced. In this case, the form depends on $n$.


\[ 
\statabs = 
\begin{dcases}
\frac{4(n-1)}{n^2}\sum_{i=1}^{g}n_i \left|\bar{r}_i-\frac{n+1}{2} \right|, &\mbox{if } n \mbox{ is even;} \\
\frac{4}{n+1}\sum_{i=1}^{g}n_i \left|\bar{r}_i-\frac{n+1}{2} \right|, &\mbox{if } n \mbox{ is odd.} \\
\end{dcases}  
\]

We call the process to calculate the $h$-test statistic in this setting $\KWA$.

\begin{theorem} \label{thm:abssensi}
The sensitivity of $\statabs$ is bounded by 8.
\end{theorem}

See Appendix \ref{sec:kw_abs_sens} for a proof of Theorem \ref{thm:abssensi}.

The absolute value private Kruskal-Wallis algorithms are similar to Algorithms $\privKW$ and $\complete$, and we will refer to them as $\privKWA$ and $\completeA$. There are only minor differences between Algorithms $\privKW$ and $\privKWA$: we use $\KWA(\data)$ instead of $\KW(\data)$ in the calculation of the non-private test statistic and we use a sensitivity of $8$ rather than $87$ in the addition of the Laplace noise as per Theorem \ref{thm:abssensi}. There are similarities between Algorithms $\complete$ and $\completeA$: we use $\privKWA$ rather than $\privKW$ to calculate the private test statistic and we cannot use a $\chi^2$ approximation of the null distribution. See Appendix \ref{sec:kw_abs_t1} for a note on the Type I error rate of $\privKWA$.

\begin{theorem}
Algorithm $\KWA$ and $\completeA$ are $\epsilon$-differentially private.
\end{theorem}

\begin{proof}
The proof is identical to the proofs for Algorithms $\KW$ and $\complete$ (Theorems \ref{thm:pKW} and \ref{thm:pcomp}).
\end{proof}


\begin{comment}
\begin{algorithm}
\DontPrintSemicolon
\algrule
\textbf{Algorithm} $\KWA$ \textbf{:} Absolute Value Kruskal-Wallis Test Statistic Calculation\;
\algrule
\KwIn{$\data$}
\Begin{
    $g \longleftarrow \textup{the number of groups in database } \data $\;
    $\bar{r} \longleftarrow n(n+1)/2$ \;
    Order the data by increasing $v_i$\;
    \For{group $i$ of $\data$}{
        \For{data point $j$ in group $i$}{
        $r_{ij} \longleftarrow \textup{the rank of the observation}$\;
        }
        $n_i \longleftarrow \textup{the size of group }i$\;
        $\bar{r}_{i} \longleftarrow \Big(\sum_{j=1}^{n_i}r_{ij}\Big)/n_i$
    }
    $\statabs:=(n-1)\frac{\sum_{i=1}^{g}n_i|\bar{r}_i-\bar{\bar{r}}|}{\sum_{i=1}^{g}\sum_{j=1}^{n_i}|r_{ij}-\bar{\bar{r}}|} $
}
\KwOut{$\statabs$}
\algrule
\label{alg:kwa}
\end{algorithm}
\end{comment}

==> appendices/KW_Square_type_1.tex <==
The question arises: what if the (public) number of groups is "inaccurate:" $\data$ contains empty groups. Are our results still valid if we run the test with too many groups?

Let $g_r$ be the number of groups such that $n_i >0$; it follows that $g_r \leq g$. When we generate the null distribution in the public setting, we need $g_r-1$ for the degrees of freedom in the $\chi^2$ distribution. However, in the differentially private setting, $g_r$ is private information and so it cannot be used to generate the private null distribution. 

But since $g_r \leq g$, for the same $\alpha$, the critical values of $\chi^2(g-1)$ are always larger than those of $\chi^2(g_r-1)$. Thus, $$\Pr[Z>z'^*]<\Pr[Z>z^*]=\Pr[Z'>z'^*]=\alpha,$$ where $Z,\ Z'$ are random variables when $g_r<g$ and $g_r = g$, respectively, and $z^*, \ z'^*$ are critical values for the distributions of $Z$ and $Z'$, respectively.

Therefore, assuming that all $g$ groups have elements and using $g$ to generate the null distribution will make the type I error smaller, and thus our results are valid (but will cause some power loss).

==> figures/new_task_crit_val_table.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Fri Jul  6 10:24:24 2018
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrr}
  \hline
 & NR\_min & 0.0595 & .03475 & .0199 & .01495 \\ 
  \hline
1 & 10.000 & 5.632 & 5.947 & 6.314 & 6.563 \\ 
  2 & 20.000 & 4.566 & 4.881 & 5.247 & 5.497 \\ 
  3 & 30.000 & 4.059 & 4.374 & 4.740 & 4.990 \\ 
  4 & 40.000 & 3.748 & 4.063 & 4.430 & 4.679 \\ 
  5 & 50.000 & 3.533 & 3.848 & 4.215 & 4.464 \\ 
  6 & 100.000 & 2.990 & 3.305 & 3.671 & 3.921 \\ 
  7 & 200.000 & 2.600 & 2.915 & 3.281 & 3.530 \\ 
  8 & 300.000 & 2.425 & 2.740 & 3.107 & 3.356 \\ 
  9 & 400.000 & 2.321 & 2.636 & 3.003 & 3.252 \\ 
  10 & 500.000 & 2.250 & 2.565 & 2.931 & 3.181 \\ 
  11 & 1000.000 & 2.073 & 2.388 & 2.755 & 3.004 \\ 
   \hline
\end{tabular}
\end{table}

